A Business Goal Driven Approach for Understanding and Specifying Information Security Requirements

In this paper we present an approach for specifying and prioritizing information security requirements in organizations. It is important to prioritize security requirements since hundred per cent security is not achievable and the limited resources available should be directed to satisfy the most important ones. We propose to link explicitly security requirements with the organization's business vision, i.e. to provide business rationale for security requirements. The rationale is then used as a basis for comparing the importance of different security requirements. A conceptual framework is presented, where the relationships between business vision, critical impact factors and valuable assets (together with their security requirements) are shown.

==> approach.tex <==
%****************************************************************************
% Section approach 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $Id: costs.tex,v 1.1 2005/06/22 15:04:02 wombachera Exp $
% 
% $Log: costs.tex,v $
% Revision 1.1  2005/06/22 15:04:02  wombachera
% no message
%
%
%****************************************************************************
\label{Sec:approach}


A security requirement specification tells what should be secured and why. It identifies the organizations' needs with respect to security. Considere, for example, the differences between the needs of a university and those of a cryptographic organization. The university fosters scholarship and open research: papers, discoveries, and work are available to the general public as well as to other academics. The cryptographic organization, on the other hand, prizes secrecy. The university will need to protect the integrity and confidentiality of the data, such as grades, on its systems. It might also want to ensure that the system is available via the Internet so that students, faculty, and other researchers have access to information. The cryptographic organization, though, will emphasize confidentiality of all its work. 

When an organization wants to secure its system, it must first determine what requirements to meet. Given that organizations  normally have limited resources to protect its assets, it is equally important to determine which requirements are more important and thus should be prioritized. To achieve this, we propose to use  a conceptual framework where security requirements are linked to the unique business drivers of the organization in question.  Figure \ref{Fig:influence_diagram} portrays the conceptual framework.  Business vision are high level business goals the organization has. Critical Impact Factors (CIFs) identify what will be the business impacts if security requirements are violated. Valuable assets and their security requirements are inventories of security requirements. Valuable assets and their security requirements have an effect on the CIFs and the CIFs in turn impact the accomplishment of the organization's business vision. In other words, we can use organization's business vision to prioritize the CIFs, which further can be used to prioritize the security requirements. To achieve that, three subsequent steps need to be taken. Firstly we need to enumerate valuable assets and their security requirements. Secondly, an organization's CIFs and business vision need to be defined. Thirdly, security requirements shall be linked with CIFs and business vision. We will discuss them in detail. 

\epsfigureP{pics/influence_diagram.eps}{0.6}
{Linking security requirements with business vision via CIF.}
{Fig:influence_diagram}{htb}

\subsection{The business vision}


%At a strategic level, each organization has its unique business vision that defines the goal the organization wants to achieve. The business vision is normally defined  by taking into consideration: the industry in which the organization competes or exists, an understanding of the organization's peers,  problems, barriers, or challenges to the organization, and possibly other factors. For example, consider an organization that produces metal. As a member of the production industry, the organization inherits vision such as "improve operational efficiency". Consider a new online book store, its business vision would include "deliver trusted service". Information security eventually is about protecting information from a wide range of threats in order to ensure business continuity and minimize business damages so that the business vision of the organization can be accomplished. Each organization has its business vision, explicitly or implicitly. We therefore consider it is safe to assume that the business vision of the organization is already established. 

Each organization has its own unique business vision that defines the
very principles of how the business wants to achieve its goals. This 
vision, moreover, often changes over time to reflect changing
circumstances.
Notwithstanding this diversity, scholars in business administration have
identified certain ``paterns'' in the business vision of leading firms.
In this paper, we use the well-known \emph{value disciplines} identified
by Treacy and Wiersema~\cite{treacy.wiersema.hbr93,treacy.wiersema.dml97}
as a frameworks for understanding the business vision.

Treacy and Wiersema argue that there are three generic ways a business
can differentiate itself from the competition, which they call {\em
operational excellence}, \emph{customer intimacy}, and \emph{product leadership}. Each
of these three value disciplines aims at creating distinguishing value
for customers in a different way. A company striving for operational
excellence focuses on offering its products with the least possible hassle
(usually, at the lowest cost) to its customers. A customer intimacy company aims at 
delivering exactly what its customers want by investigating the needs of a narrow market and customizing its offerings to this market. Finally, a product leader aims at delivering radically innovative products that create an unbridgable gap with the competition.

Each of the three value disciplines leads to a radically different
operating model for the company: the culture, processes, management systems and
IT systems of the company. For instance, while operational excellence
calls for highly standardized business processes, the customer intimacy
discipline requires just the opposite: to meet customer requirements, business
processes should be as flexible as possible. Security requirements should be
likewise aligned with the requirements imposed upon culture, processes and
management systems by the value discipline choosen.

\subsection{Identifying the critical impact factors}
When security incidents happen, they may lead to damage to organizations. Critical impact factors (CIFs) are the indicators about what kind of damage the security incidents incur to the organization. They can include those within the control of the organization, as well as some that the organization may not be able to fully control (e.g., legal liability, finance losses and reputational damage).

The identification activity of CIFs is also referred as business impact analysis (BIA): it is important to remark the difference between BIA and risk analysis. 

BIA identifies the critical business functions within the organization and determines the effect of external and internal CIFs upon the various parts of organization, using a combination of relevant literature study and specific case studies in the organizations.

Risk analysis involves identifying the most probable threats to an organization and analyzing the related vulnerabilities of the organization to those threats.

Figure \ref{Fig:CIFs} illustrate an example list of critical impact factors. 

\epsfigureP{pics/CIFs.eps}{0.6}
{An example of Critical Impact Factors.}
{Fig:CIFs}{htb}

\subsection{Selecting valuable assets and security requirements}
The business vision can be used to guide the selection of valuable assets. Surely, the assets that are critical for accomplishing the business vision are the valuable ones for the organizations. For example, a financial service company that focuses on customer intimacy will consider its customer relationship management (CRM) systems as extremely valuable, while a financial service company that focuses at product leadership will likely value its systems for developing new financial products even higher.

Information security has been defined as encompassing systems and procedures designed to ensure the confidentiality, integrity and availability \footnote{some authorities treat communication security issues such as non-repudiation and privacy related issues such as anonymity as additional aspects of security} of an organization's critical information and technical assets. Information assets represent the data and information, in either physical or electronic from, that is critical to the organization. Technical assets represent those assets that support the storage, transmission, and processing of data and information and therefore are important to transforming data and information to be used by the organization. People can be an asset to the organization as well for similar reason -- they can be a primary way of storing, transporting, or processing data.

So, IT security is about safeguard certain desired properties. The core of computer and information security is widely regarded as the preservation of three factors: confidentiality (ensuring that information is accessible only to those authorized to access), integrity (safeguarding the accuracy and completeness of information and processing methods) and availability (ensuring that authorized users have access to information and associated assets when required) \cite{Furnell_2005_Security}.

\epsfigureP{pics/asset_classification.eps}{0.6}
{A simple ontology of asset and security property.}
{Fig:asset_classification}{htb}

Figure \ref{Fig:asset_classification} depicts a simple ontology of asset and the security properties that are in the scope. Such an ontology can be used as a starting point to structure assets and their security properties. It is a minimum set and can be extended. For instance, some will include privacy issues like anonymity  as a security property too. Using such an ontology, the assets and their security properties can be structured accordingly. Figure \ref{Fig:example_asset} gives an example. 

\epsfigureP{pics/example_asset.eps}{0.6}
{An example of assets and their security properties.}
{Fig:example_asset}{htb}


\subsection{Prioritizing security requirements}


\epsfigureP{pics/example_impact_link.eps}{0.6}
{An example of linking asset security requirement with business vision via CIFs.}
{Fig:example_impact_link}{htb}

To further elaborate the relations between security requirements and the business vision, the connection between them can be established via the linkage of CIFs. Figure \ref{Fig:example_impact_link} provides an example of such linkage for a production company. In this example, the organization is stating that any compromise to "availability" of the "control system"  has "critical impact" to "loss of productivity", which in turn has "critical impact" to the organization's vision "improve operational efficiency". The impact severity can be categorized according to the organization's needs. An example categorization can be \emph{critical impact}, \emph{marginal impact}, and \emph{negligible impact}. In this way, each security requirements can be connect its CIFs and the CIFs further to business vision.

Using the impact diagram like figure \ref{Fig:example_impact_link}, it is possible to categorize and  prioritize the different security requirements.  Requirements that have "critical impacts"  on CIFs, which have "critical impacts" on business vision, should be considered of most importance. These requirements shall be satisfied first if the resources (time, money, manpower etc.) are limited. In this example, it means  for the production company, it is more important to mitigate threats to the control system's availability  than for instance, threats to the control system's confidentiality. It is possible that one requirement may be linked to more than one CIFs. When that happens the overall significance of that security requirement can be determined by a number of ways. For example, one can choose the maximum impact level, e.g. if control system's availability not only "critical impacts" on loss of productivity but also has "marginal impact" on reputation damage, the overall impact should be "critical impacts". Alternatively, one can choose the average impact level. The organization shall decide which combination methods best reflects its situation.  

The reason why we use CIFs to link critical assets and their security requirements with business goals is twofold. Business goals typically reside at strategic level. When the business goals are outlined, the stakeholders do not normally have a security focus in mind. The Critical Impact Factors on the other hand, reflect the business implication when security is compromised. It is of course possible to directly connect assets' security requirements with business goals. But then the shift of focus from pure technical level security concern to strategical level business concern  seems abrupt. The introduction of CIFs makes the shift smooth and the line of reasoning easier to follow. 

Once the requirements are categorized and prioritized. Other techniques, like attacks trees or misuse cases can be used to explore all possible threats and attack paths  that would lead to the violation of security properties. In this example, it is to find out how the control system's availability can be compromised.  Our approach is complementary to this line of work, in the sense that we provides a business grounded rational for why certain security requirements are important while others are not. 

==> related_research.tex <==
%****************************************************************************
% Section literature
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% $Id: discussion.tex,v 1.2 2005/07/06 14:17:53  Exp $
% 
% $Log: discussion.tex,v $
% Revision 1.2  2005/07/06 14:17:53  
% no message
%
%
%%
%****************************************************************************
\label{Sec:related_research}

There exists a number of security standards, among which COBIT (Control Objectives for Information and related Technology)~\cite{cobit} and BS7799~\cite{bs7799} are of particular relevance to our work. COBIT is an international de-facto standard for information control and IT risk management, addressing IT governance and control practices. It provides a reference business-oriented framework for management, users and control and security auditors. COBIT defines control objectives but does not provide guidelines on how to reach the objectives. BS7799 (originally published in 1995) is strictly focused on IT security and it is divided into two parts. The first part \textit{Code of Practice for Information Security Management} became an official ISO standard, ISO 17799, in 2000. It contains general security guidelines including policies, practices, procedures, organizational structures and software functions. The second part \textit{Information Security Management - Specifications} became a ISO standard, ISO 27001, in 2005. It contains technical requirements. ISO17799/27001  addresses company's security from a best practice point of view, which does not provide  any answer to why certain security mechanisms are in place for a particular organization. Both COBIT and ISO17799 however, do not define guidelines on how to prioritize in a proper way the company assets and their security properties. 

Our approach is also related to the work of security requirement modeling. Sinder and Opdahl \cite{Sindre_2005} suggested to have negative use cases or scenarios in connection with security. Yu and Liu ~\cite{Yu_2000_trust}  in their work shows actors and misactors having contradictory goals in an extension of $i^{*}$ diagrams \cite{Mylopoulos_1999}. Links such as "break" or "hurt" can show how an attack prevents the legitimate users from reaching their goals, or how countermeasures can thwart an attacks. This line of work focuses on how to model threat, including the threat actors and their attack paths. Our approach on the other hand, focuses on providing business rationale for explaining why certain security requirements exist in the first place as well as explaining why some security requirements are more important than others. Our approach can be combined with the modeling work. First, the security requirements are ranked using our approach. Next, for the prioritized security requirements, misuse case or attack trees \cite{Schneier_2000} can be use to model how  attacks that will violate the security requirements could actually happen.

Finally, our work is also related to the work of security risk assessment. Traditionally, in risk assessment methodologies, e.g. OCTAVE ~\cite{octave} (Operationally Critical Threat, Asset and Vulnerability Evaluation), risk of each threat is determined by the impact of the threat once it happens and how likely it will happen [REF]. For the impact, a severity level (e.g. high, low or medium) is assigned. What often happens is that the severity level is assigned based on the person's own experience without explicit rationale. Our approach can enhance this process because it provides an explicit tie to the organization's business drivers. 

